A Semantics for Belief in Simplicial Complexes

We provide novel semantics for belief using simplicial complexes. In our framework, belief is a KD45 modality that satisfies "knowledge implies belief" ("If you know phi, then you believe phi"); in addition, we adopt the (standard) assumption that each facet in our simplicial models contains exactly one vertex for each agent. No existing model of belief in simplicial complexes that we are aware of is able to satisfy all of these conditions without trivializing belief to coincide with knowledge. We establish a truth-preserving correspondence between our simplicial framework and standard relational models for knowledge and belief; this involves, notably, proving that all relational models can be simulated using proper relational models, a result of independent interest. Finally, we apply these results to provide a simple axiomatization.

==> eptcsdata.tex <==
\providecommand{\firstpage}{173}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.10}{10.4204/EPTCS.447.10}}

